Training Object Detectors on Synthetic Images Containing Reflecting Materials

One of the grand challenges of deep learning is the requirement to obtain large labeled training data sets. While synthesized data sets can be used to overcome this challenge, it is important that these data sets close the reality gap, i.e., a model trained on synthetic image data is able to generalize to real images. Whereas, the reality gap can be considered bridged in several application scenarios, training on synthesized images containing reflecting materials requires further research. Since the appearance of objects with reflecting materials is dominated by the surrounding environment, this interaction needs to be considered during training data generation. Therefore, within this paper we examine the effect of reflecting materials in the context of synthetic image generation for training object detectors. We investigate the influence of rendering approach used for image synthesis, the effect of domain randomization, as well as the amount of used training data. To be able to compare our results to the state-of-the-art, we focus on indoor scenes as they have been investigated extensively. Within this scenario, bathroom furniture is a natural choice for objects with reflecting materials, for which we report our findings on real and synthetic testing data.

==> viscom-header.tex <==
% extensions to realize
%- \myfigure command with label
%- \etc, \ie, \eg ...



\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xifthen}
\usepackage{pgfplots}
\usepackage{tikz,graphicx}
\usetikzlibrary{arrows}
\usetikzlibrary{colorbrewer}
\usepgfplotslibrary{colorbrewer}
\newcommand{\textred}[1]{\textcolor{red}{#1}}
\newcommand{\textgreen}[1]{\textcolor{green}{#1}}
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}

\tikzset{>=latex}

\newcommand{\point}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\todo}[2][]{%
  \ifthenelse{\equal{#1}{}}
    {{\color{red}TODO:~#2}}
    {{\color{red}TODO~[#1]:~#2}}
}

\makeatletter
\newcommand{\mypart@star}[2]{\part*{#1}\label{#2}}
\newcommand{\mypart@nostar}[3][]{\part[#1]{#2}\label{#3}}
\newcommand{\mychapter@star}[2]{\chapter*{#1}\label{#2}}
\newcommand{\mychapter@nostar}[3][]{\chapter[#1]{#2}\label{#3}}
\newcommand{\mysection@star}[2]{\section*{#1}\label{#2}}
\newcommand{\mysection@nostar}[3][]{\section[#1]{#2}\label{#3}}
\newcommand{\mysubsection@star}[2]{\subsection*{#1}\label{#2}}
\newcommand{\mysubsection@nostar}[3][]{\subsection[#1]{#2}\label{#3}}
\newcommand{\mysubsubsection@star}[2]{\subsubsection*{#1}\label{#2}}
\newcommand{\mysubsubsection@nostar}[3][]{\subsubsection[#1]{#2}\label{#3}}
\newcommand{\myparagraph@star}[2]{\paragraph*{#1}\label{#2}}
\newcommand{\myparagraph@nostar}[3][]{\paragraph[#1]{#2}\label{#3}}
\newcommand{\mysubparagraph@star}[2]{\subparagraph*{#1}\label{#2}}
\newcommand{\mysubparagraph@nostar}[3][]{\subparagraph[#1]{#2}\label{#3}}

\newcommand{\mypart}{\@ifstar{\mypart@star}{\mypart@nostar}}
\newcommand{\mychapter}{\@ifstar{\mychapter@star}{\mychapter@nostar}}
\newcommand{\mysection}{\@ifstar{\mysection@star}{\mysection@nostar}}
\newcommand{\mysubsection}{\@ifstar{\mysubsection@star}{\mysubsection@nostar}}
\newcommand{\mysubsubsection}{\@ifstar{\mysubsubsection@star}{\mysubsubsection@nostar}}
\newcommand{\myparagraph}{\@ifstar{\myparagraph@star}{\myparagraph@nostar}}
\newcommand{\mysubparagraph}{\@ifstar{\mysubparagraph@star}{\mysubparagraph@nostar}}
\makeatother

